KCRL: Krasovskii-Constrained Reinforcement Learning with Guaranteed Stability in Nonlinear Dynamical Systems

Learning a dynamical system requires stabilizing the unknown dynamics to avoid state blow-ups. However, current reinforcement learning (RL) methods lack stabilization guarantees, which limits their applicability for the control of safety-critical systems. We propose a model-based RL framework with formal stability guarantees, Krasovskii Constrained RL (KCRL), that adopts Krasovskii's family of Lyapunov functions as a stability constraint. The proposed method learns the system dynamics up to a confidence interval using feature representation, e.g. Random Fourier Features. It then solves a constrained policy optimization problem with a stability constraint based on Krasovskii's method using a primal-dual approach to recover a stabilizing policy. We show that KCRL is guaranteed to learn a stabilizing policy in a finite number of interactions with the underlying unknown system. We also derive the sample complexity upper bound for stabilization of unknown nonlinear dynamical systems via the KCRL framework.

==> Arxiv/6-RelatedWork.tex <==
This paper connects to a broad set of literature in RL and control.

\textit{Model-based RL in dynamical systems.} There has been a flurry of studies that consider model-based RL in dynamical systems due to their superior sample efficiency, task generalization and interpretable guarantees~\cite{recht2019tour}. The main focus has been on learning the system dynamics and providing performance guarantees in finite-time for both linear \cite{simchowitz2020naive} (and references within),
%~\cite{oymak2018non,sarkar2019finite,simchowitz2020naive,faradonbeh2020adaptive,lale2020logarithmic} 
and nonlinear systems~\cite{kakade2020information,lale2021model}. While deriving these performance guarantees, the formal finite-time stability guarantees are also derived for linear systems~\cite{faradonbeh2018finite}. However, these guarantees have only been \textit{assumed to hold} with a stabilizing oracle for nonlinear systems~\cite{kakade2020information,lale2021model}. Therefore, our work completes an important part of the picture in finite-time stabilization of dynamical systems. 

\textit{Control Theory.} Our work is related to the Krasovskii's method~\cite{feijer2009krasovskii} and contraction analysis~\cite{lohmiller1998contraction}, which can be viewed as a specific way of constructing a Lyapunov function. More broadly, there are a large body of tools in control theory that synthesize controllers that are stable, e.g., passivity theory and feedback linearization~\cite{slotine1991applied}.
% , model-predictive control (MPC)~\cite{rawlings2017model}
In the context of these works, our contribution can be viewed as bridging one of these classical tools with policy learning in RL, where the system model is unknown.

\textit{Lyapunov-based Policy Learning.} Lyapunov theory is a systematic framework to analyze the stability of a control system. The core idea is to identify a Lyapunov function of the state, with negative derivative along system trajectories. 
Using Lyapunov functions in RL was first introduced by~\cite{perkins2002lyapunov}, but the work did not discuss how to find a candidate Lyapunov function in general. 
% except for a case-by-case construction. 
A set of recent works including~\cite{chow2018lyapunov,richards2018lyapunov,chang2019neural,jin2020neural} have attempted to address this challenge by jointly learning the policy and the Lyapunov function.
%where \cite{chow2018lyapunov} uses linear programming and others parameterize the Lyapunov function as neural networks. 
Our goals and approaches are different. We use a principled framework to \textit{construct} (rather than learn) the Lyapunov function, and design the policy learning such that the stability conditions are met. In this sense, \cite{shi2021stability} is most related to our work. It considers a particular power system model and proposes model-free monotonic policies to stabilize the system. However, their model assumption is specific to power systems, whereas our work considers general nonlinear systems. 

\textit{Safe RL.} The goal of safe RL is to learn a policy that avoids entering unsafe regions, rather than requiring a policy to have attractive or bounded behavior. Various methods have been proposed to ensure safety in RL, %see~\cite{garcia2015comprehensive} for a survey of this topic. In addition, many recent works focus on ensuring safety via control-theoretic methods 
such as using control barrier functions~\cite{taylor2020learning}, Hamilton-Jacobi safety analysis~\cite{fisac2019bridging}, and MPC as a safety filter~\cite{hewing2020learning}. We note that safety does not imply stability and vice visa, and our main focus in this paper is to learn an RL policy with the stability guarantee.
%In some sense, stability is a more stringent requirement as it can lead to asymptotic safety satisfaction.



% \textit{Reinforcement Learning for Power Systems.} Voltage control is a fundamental problem in the safe and efficient operation of power systems under high penetration of renewables. Our work contributes to a growing line of papers that use RL for voltage control~\cite{chen2021reinforcement,wang_data-driven_2020,wang_safe_2020}, see \cite{chen2021reinforcement} for a recent review. As pointed out in  \cite{chen2021reinforcement}, one of the key issues in RL for power system control is the lack of a stability guarantee, and our work makes a step toward addressing this issue by providing a formal stability guarantee on the learned policy. In particular, our experiments compare against~\cite{wang_data-driven_2020}, which uses standard multi-agent DDPG for voltage control. Closest to the spirit to our paper is~\cite{Cui2021a}, which proposes a stable RL approach for frequency control via a Lyapunov approach. However, their approach depends on the specific Lyapunov function for the application, while our method can be applied to the broader class of systems 
% with Krasovskii's method to construct the Lyapunov function.

%used \adam{We should probably say a bit more about the specific related work comparison in the case of voltage control...highlight baosen's work}
%for example \cite{xu_optimal_2020,wang_data-driven_2020,wang_safe_2020,duan_deep-reinforcement-learning-based_2020,cao_multi-agent_2020,liu2020two} [\todo{too much?}], 
